GRASP: A Rehearsal Policy for Efficient Online Continual Learning

Continual learning (CL) in deep neural networks (DNNs) involves incrementally accumulating knowledge in a DNN from a growing data stream. A major challenge in CL is that non-stationary data streams cause catastrophic forgetting of previously learned abilities. A popular solution is rehearsal: storing past observations in a buffer and then sampling the buffer to update the DNN. Uniform sampling in a class-balanced manner is highly effective, and better sample selection policies have been elusive. Here, we propose a new sample selection policy called GRASP that selects the most prototypical (easy) samples first and then gradually selects less prototypical (harder) examples. GRASP has little additional compute or memory overhead compared to uniform selection, enabling it to scale to large datasets. Compared to 17 other rehearsal policies, GRASP achieves higher accuracy in CL experiments on ImageNet. Compared to uniform balanced sampling, GRASP achieves the same performance with 40% fewer updates. We also show that GRASP is effective for CL on five text classification datasets.

==> figures/front_fig.tex <==

\begin{figure}[t]
  \centering
   \includegraphics[width=0.45\linewidth]{images/compute_replay_updated.png}
   \caption{The GRASP rehearsal policy outperforms 17 others in online continual learning. %Compute specifies the number of gradient descent updates across rehearsal cycles. 
   GRASP achieves the best accuracy of the popular uniform balanced policy with $40\%$ speedup i.e., $40\%$ fewer gradient descent updates.      
   }
   \label{fig:summary}
\end{figure}

==> figures/memory_compute.tex <==
\begin{figure}[h]
  \centering

\begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/memory_comparison_updated.png}
         \caption{Impact of Memory Constraints}
         \label{fig:memory}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/compute_comparison_updated.png}
         \caption{Impact of Compute Constraints}
         \label{fig:compute}
     \end{subfigure}
     \hfill
   \caption{Performance of various rehearsal policies under varied memory and compute constraints in CIL on ImageNet-300 using SIESTA and latent rehearsal. Reported accuracy is the final top-1 accuracy ($\%$) on all 300 ImageNet classes.
   \label{fig:mem_com}}
   %\vspace{-2em}
\end{figure}


==> figures/relative_train_time_AND_drift.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/grasp_barplot.png}
        \caption{Relative Training Time}
        \label{fig:relative_train_time}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/grasp_drift.png}
        \caption{Representation Drift}
        \label{fig:drift}
    \end{subfigure}
    \hfill
    \caption{(a) Existing methods require significantly longer training time than GRASP. %\jc{This part highlights efficiency; could be moved before other results. } \yh{done} 
    (b) The representation drift of old classes while learning new classes in a stream of two tasks. GRASP reduces the representation drift. %\jg{I put both figures in 1. Yousuf, please revise the caption.}
    }
    \label{fig:relative_train_time_and_drift}
\end{figure}

==> figures/replays.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.45\linewidth]{images/grasp_veridical_replay.png}
   \caption{ImageNet-1K learning curves of GRASP and uniform balanced policies in CIL. Both use SIESTA. 
   }
   \label{fig:learning_curve}
\end{figure}

==> figures/time.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.45\linewidth]{images/time_replay_updated.png}
   \caption{The GRASP rehearsal policy matches uniform balanced's best accuracy while providing $36\%$ speedup in training time for end-to-end CIL on ImageNet-1K with SIESTA and latent rehearsal.
   }
   \label{fig:time}
\end{figure}

==> tables/compute.tex <==
\begin{table}[h] 
  \caption{
   \textbf{Compute Constraint Analysis.} GRASP vs. uniform balanced under various compute constraints in CIL on \textbf{ImageNet-1K} with SIESTA using latent rehearsal. %Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote accuracy ($\%$) on new, old, and all classes, respectively, averaged over rehearsal cycles. $\alpha$ is the final accuracy ($\%$) on all classes.
   Reported number of updates is in million.
   }
  \centering
     \begin{tabular}{lccccc}
     \hline
     \textbf{Method} & \textbf{Updates (M)} & $\mu_{N} \uparrow$ & $\mu_{O} \uparrow$ & $\mu_{A} \uparrow$ & $\alpha \uparrow$ \\
     \hline
     %Upper Bound & --- & --- & --- & --- & $62.12$ \\
     %\hline
      & $0.76$ & $65.12$ & $68.40$ & $67.81$ & $59.10$ \\
     Uniform Bal & $1.02$ & $66.38$ & $69.07$ & $68.58$ & $60.28$ \\
     & $1.28$ & $66.96$ & $69.36$ & $68.93$ & $60.79$ \\
     & $1.53$ & $67.40$ & $69.61$ & $69.20$ & $61.10$ \\
     \hline
     & $0.76$ & $66.07$ & $69.44$ & $68.78$ & $60.00$ \\
     GRASP & $1.02$ & $67.15$ & $70.06$ & $69.57$ & $61.36$ \\
     & $1.28$ & $68.30$ & $70.46$ & $70.11$ & $61.93$ \\
     & $1.53$ & $68.69$ & $70.54$ & $70.26$ & $62.66$ \\
     \hline
    \end{tabular}
%\caption{
%   \textbf{Compute Constraint Analysis.} GRASP vs. uniform balanced under various compute constraints in CIL on \textbf{ImageNet-1K} with SIESTA using latent rehearsal.  $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy ($\%$) on new, old, and all classes, respectively, averaged over rehearsal cycles. $\alpha$ is the final top-1 accuracy ($\%$) on all classes.}
    
\label{tab:compute}
\end{table}

==> tables/coreset.tex <==
\begin{table*}[t!]
  \centering
     \begin{tabular}{l|rrrrrr|rrrrrr}
     \hline
     \multicolumn{1}{c|}{\textbf{Method}} &
     \multicolumn{6}{c|}{\textbf{Unconstrained Memory}} &
     \multicolumn{6}{c}{\textbf{Constrained Memory}} \\
      & $\mu_{N}(\uparrow)$ & $\mu_{O}(\uparrow)$ & $\mu_{A}(\uparrow)$ & $\alpha(\uparrow)$ & $\mathcal{C}(\downarrow)$ & $T(\downarrow)$ & $\mu_{N}(\uparrow)$ & $\mu_{O}(\uparrow)$ & $\mu_{A}(\uparrow)$ & $\alpha(\uparrow)$ & $\mathcal{C}(\downarrow)$ & $T(\downarrow)$ \\
     \hline
     OCS & $83.15$ & $74.27$ & $74.93$ & $70.36$ & -- & $7.34$ & $82.51$ & $73.46$ & $74.13$ & $69.01$ & -- & $7.14$ \\
     GSS & $\mathbf{87.91}$ & $73.97$ & $75.04$ & $70.25$ & -- & $11.60$ & $\mathbf{88.01}$ & $74.34$ & $75.38$ & $70.47$ & -- & $8.85$ \\
     Grad Matching & $85.78$ & $75.72$ & $76.48$ & $72.20$ & -- & $12.71$ & $85.91$ & $75.97$ & $76.71$ & $72.36$ & -- & $12.93$ \\
     %Bi-level & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
     \textbf{GRASP} & $73.08$ & $\mathbf{78.18}$ & $\mathbf{77.75}$ & $\mathbf{73.96}$ & -- & $\mathbf{0.13}$ & $73.61$ & $\mathbf{78.25}$ & $\mathbf{77.88}$ & $\mathbf{73.71}$ & -- & $\mathbf{0.13}$ \\
     \hline
    \end{tabular}
  \caption{
   \textbf{Comparison with Coreset-based Methods on ImageNet-150.} This is based on memory-bound CIL with SIESTA. Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy ($\%$) on new, old, and all classes, respectively, averaged over incremental batches, and $\alpha$ is the final top-1 accuracy ($\%$) on all classes. $\mathcal{C}$ and $T$ denote training FLOPs and training time in hours, respectively.
   }
  \label{tab:coreset}
\end{table*}

==> tables/cub.tex <==

\begin{table}[h]
  \caption{ 
  \textbf{CUB-200 Results.}
   Comparison between GRASP and uniform balanced in CIL on CUB-200 with SIESTA and latent rehearsal. Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote accuracy ($\%$) on new, old, and all classes respectively averaged over rehearsal sessions. And $\alpha$ is the final accuracy ($\%$) on all classes. Accuracy is averaged over 6 runs.}
  \centering
     \begin{tabular}{l|cccc|cccc}
     \hline
     \multicolumn{1}{c|}{\textbf{Method}} &
     \multicolumn{4}{c|}{\textbf{Unbounded Memory}} &
     \multicolumn{4}{c}{\textbf{Bounded Memory}} \\
     
      & $\mu_{N} \uparrow$ & $\mu_{O} \uparrow$ & $\mu_{A} \uparrow$ & $\alpha \uparrow$ & $\mu_{N} \uparrow$ & $\mu_{O} \uparrow$ & $\mu_{A} \uparrow$ & $\alpha \uparrow$ \\
     %\hline
     %Upper Bound & --- & --- & --- & $58.48$ & --- & --- & --- & $58.48$ \\
     \hline
     Uniform Bal & $57.56$ & $58.69$ & $58.58$ & $54.90$ & $56.43$ & $57.45$ & $57.34$ & $51.71$ \\
     \textbf{GRASP} & $\mathbf{59.35}$ & $\mathbf{60.12}$ & $\mathbf{60.14}$ & $\mathbf{56.06}$ & $\mathbf{58.68}$ & $\mathbf{58.79}$ & $\mathbf{59.04}$ & $\mathbf{53.06}$ \\
     \hline
    \end{tabular}
  \label{tab:cub}
\end{table}


==> tables/iid_cl.tex <==
\begin{table}[t]
  % \caption{
  %  \textbf{IID Results.} Comparison between GRASP and uniform class-balanced rehearsals in IID continual learning on \textbf{ImageNet-1K}. Both methods perform latent rehearsal under compute and memory constraints. Uniform class-balanced rehearsal is referred as Uniform to save space.
  %  Here $\mu$ denotes top-1 accuracy on all classes averaged over rehearsal cycles. And $\alpha$ is the final top-1 accuracy on all classes. The $(\uparrow)$ indicates high value is desirable.}
  % \label{tab:iid}
  \centering
     \begin{tabular}{lrr}
     \hline
     Method & $\mu (\uparrow)$ & $\alpha (\uparrow)$ \\
     \hline
     Offline & --- & $62.12$ \\
     \hline
     Uniform & $60.35$ & $61.56$ \\
     GRASP & $\mathbf{61.51}$ & $\mathbf{63.12}$ \\
     \hline
    \end{tabular}
  \caption{
   \textbf{IID Results.} Comparison between GRASP and uniform class-balanced rehearsals in IID continual learning on \textbf{ImageNet-1K}. Both methods perform latent rehearsal under compute and memory constraints. Uniform class-balanced rehearsal is referred as Uniform to save space.
   Here $\mu$ denotes top-1 accuracy on all classes averaged over rehearsal cycles. And $\alpha$ is the final top-1 accuracy on all classes. The $(\uparrow)$ indicates high value is desirable.}
  \label{tab:iid}
\end{table}

==> tables/more_memory.tex <==
\begin{table}[t]
  \caption{
   \textbf{Memory Constraint Analysis.} GRASP vs. uniform balanced under various memory constraints in CIL on \textbf{ImageNet-1K} with SIESTA using latent rehearsal. %Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote accuracy ($\%$) on new, old, and all classes, respectively, averaged over rehearsal cycles. $\alpha$ is the final accuracy ($\%$) on all classes.
   Buffer size is reported in GB.}
  \centering
     \begin{tabular}{lccccc}
     \hline
     \textbf{Method} & \textbf{Buffer} & $\mu_{N} \uparrow$ & $\mu_{O} \uparrow$ & $\mu_{A} \uparrow$ & $\alpha \uparrow$ \\
     \hline
     %Upper Bound & --- & --- & --- & --- & $62.12$ \\
     %\hline
      & $2.01$ & $66.96$ & $69.36$ & $68.93$ & $60.79$ \\
     Uniform Bal & $1.51$ & $67.02$ & $69.34$ & $68.95$ & $60.27$ \\
      & $0.75$ & $66.25$ & $67.89$ & $67.59$ & $57.13$ \\
     %& $130000$ & $60.56$ & $60.10$ & $60.04$ & $45.68$ \\
     \hline
      & $2.01$ & $68.30$ & $70.46$ & $70.11$ & $61.93$ \\
     GRASP & $1.51$ & $68.25$ & $70.30$ & $69.96$ & $61.99$ \\
      & $0.75$ & $67.66$ & $68.95$ & $68.69$ & $58.44$ \\
     %& $130000$ & --- & --- & --- & -- \\
     \hline
    \end{tabular}

   %   \caption{
   %\textbf{Memory Constraint Analysis.} GRASP vs. uniform balanced under various memory constraints in CIL on \textbf{ImageNet-1K} with SIESTA using latent rehearsal. $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy ($\%$) on new, old, and all classes, respectively, averaged over rehearsal cycles. $\alpha$ is the final top-1 accuracy ($\%$) on all classes. Buffer size is reported in GB.}
  \label{tab:more_mem}
\end{table}

==> tables/pruning.tex <==
\begin{table}[h]
  % \caption{
  %  \textbf{Dataset Pruning Results.} Comparison between GRASP and uniform dataset pruning methods in compute and memory constrained class incremental learning on \textbf{ImageNet-1K}. Uniform balanced latent rehearsal is performed for each pruning method.
  %  Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy on new, old, and all classes respectively averaged over incremental batches. And $\alpha$ is the final top-1 accuracy on all classes. Budget refers to maximum number of samples that each method can store in the memory buffer until buffer is full. The $(\uparrow)$ indicates high value is desirable.}
  % \label{tab:pruning}
  \centering
     \begin{tabular}{lrrrrr}
     \hline
     Pruning & Budget & $\mu_{N}(\uparrow)$ & $\mu_{O}(\uparrow)$ & $\mu_{A}(\uparrow)$ & $\alpha(\uparrow)$ \\
     \hline
     Offline & --- & --- & --- & --- & $62.12$ \\
     \hline
     % & $959665$ & $67.02$ & $69.34$ & $68.95$ & $60.27$ \\
     Uniform & $479665$ & $66.25$ & $67.89$ & $67.59$ & $57.13$ \\
     & $130000$ & $60.56$ & $60.10$ & $60.04$ & $45.68$ \\
     \hline
     % & $959665$ & -- & -- & -- & -- \\
     GRASP & $479665$ & $65.92$ & $67.77$ & $67.45$ & $56.93$ \\
      & $130000$ & $60.00$ & $59.56$ & $59.45$ & $44.64$ \\
     \hline
    \end{tabular}
  \caption{
   \textbf{Dataset Pruning Results.} Comparison between GRASP and uniform dataset pruning methods in compute and memory constrained class incremental learning on \textbf{ImageNet-1K}. Uniform balanced latent rehearsal is performed for each pruning method.
   Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy on new, old, and all classes respectively averaged over incremental batches. And $\alpha$ is the final top-1 accuracy on all classes. Budget refers to maximum number of samples that each method can store in the memory buffer until buffer is full. The $(\uparrow)$ indicates high value is desirable.}
  \label{tab:pruning}
\end{table}

==> tables/replay_baselines.tex <==
\begin{table}[t!]
  \caption{ 
   \textbf{Latent Rehearsal Results for CIL with SIESTA on ImageNet Subset.} 
   Here $\mu_{A}$ denotes accuracy ($\%$) on seen classes averaged over rehearsal sessions, and $\alpha$ is the final accuracy ($\%$) on all classes. Training time $T$ is reported in hours. Due to large computational cost, ImageNet-150 is used for gradient-based methods. \jc{1. move this table below; closer to the results. 2. for better clarity split into two tables; one for ImageNet-300 and one for -150. Besides, GRASP seems to perform better on -300 than -150. potentially due to a different setup but might be challenged by reviewers. 3. conventional vs state-of-the-art: some methods belonging to sota block seem to underperform those in conventional which seems confusing. probably change the group names to focus on regular vs expensive/sophisticated. 4. could add detailed compute/memory budget in the caption.}
   }
  % \label{tab:replay_baseline}
  \centering
     \begin{tabular}{l|c|cc|cc|c}
     \hline \hline
      &
     \multicolumn{1}{c|}{\textbf{Method}} &
     \multicolumn{2}{c|}{\textbf{Unbounded Memory}} &
     \multicolumn{2}{c}{\textbf{Bounded Memory}} & 
     \multicolumn{1}{|c}{\textbf{Time}} \\
      & & $\mu_{A} \uparrow$ & $\alpha \uparrow$ & $\mu_{A} \uparrow$ & $\alpha \uparrow$ & $T \downarrow$ \\
      \hline
      \multirow{17}{*}{\rotatebox[origin=c]{90}{\textbf{\small{ImageNet-300}}}}
     & \textcolor{orange}{\emph{\textbf{Conventional}}} & & & & & \\
     & Uniform & $77.46$ & $72.26$ & $75.36$ & $68.17$ & $0.30$ \\
     & Min Confidence~\citep{gal2017deep} & $77.69$ & $72.42$ & $75.11$ & $67.79$ & $0.41$ \\
     & Min Margin~\citep{scheffer2001active} & $77.51$ & $72.59$ & $75.20$ & $67.61$ & $0.41$ \\
     & Max Loss~\citep{kawaguchi2020ordered} & $75.40$ & $68.89$ & $72.96$ & $64.55$ & $0.41$ \\
     & Min Logit Dist~\citep{chaudhry2018riemannian} & $77.36$ & $72.07$ & $75.19$ & $67.85$ & $0.41$ \\
     & $k$-Means~\citep{chaudhryER_2019} & $77.63$ & $72.56$ & $75.50$ & $68.33$ & $0.56$ \\
     & Min Rehearsal~\citep{hayes2021selective} & $75.76$ & $69.76$ & $74.87$ & $67.37$ & $0.41$ \\
     & MoF / Easy Biased~\citep{chaudhryER_2019} & $77.43$ & $71.99$ & $75.54$ & $68.60$ & $0.33$ \\
     & Hard Biased & $76.90$ & $71.89$ & $74.75$ & $67.59$ & $0.33$ \\
     %\hline
     \cline{2-7}
      & \textcolor{orange}{\emph{\textbf{State-of-the-art}}} & & & & & \\
     & Uniform Balanced~\citep{prabhu2020gdumb} & $77.52$ & $72.62$ & $75.39$ & $68.11$ & $0.32$ \\
     & Rainbow Memory~\citep{bang2021rainbow} & $74.93$ & $68.43$ & $72.73$ & $64.67$ & $3.89$ \\
     & MIR~\citep{aljundi2019online} & $77.33$ & $71.35$ & $75.30$ & $67.93$ & $1.74$ \\
     & CLIB~\citep{koh2021online} & $77.44$ & $72.21$ & $75.22$ & $67.89$ & $0.78$ \\
     & ASER~\citep{shim2021online} & $75.16$ & $69.09$ & $73.79$ & $66.09$ & $5.91$ \\
     %\hline
     \cline{2-7}
     & \textbf{GRASP} (Ours) & $\mathbf{78.39}$ & $\mathbf{73.65}$ & $\mathbf{76.12}$ & $\mathbf{69.06}$ & $0.33$ \\
     \hline \hline
     \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\small{ImageNet-150}}}}
     & \textcolor{orange}{\emph{\textbf{Gradient-based}}} & & & & & \\
     & OCS~\citep{yoononline} & $74.93$ & $70.36$ & $74.13$ & $69.01$ & $7.34$ \\
     & GSS~\citep{aljundi2019gradient} & $75.04$ & $70.25$ & $75.38$ & $70.47$ & $11.60$ \\
     & Grad Matching~\citep{campbell2019automated} & $76.48$ & $72.20$ & $76.71$ & $72.36$ & $12.71$ \\
     \cline{2-7}
     & \textbf{GRASP} (Ours) & $\mathbf{77.75}$ & $\mathbf{73.96}$ & $\mathbf{77.88}$ & $\mathbf{73.71}$ & $0.13$ \\
     \hline \hline
    \end{tabular}
  \label{tab:replay_baseline}
\end{table}

==> tables/replay_mem.tex <==
\begin{table}[t]
  % \caption{
  %  \textbf{Memory $\&$ Compute-Constrained CL.} Comparison between GRASP and uniform class-balanced rehearsals in compute and memory constrained class incremental learning on \textbf{ImageNet-1K}. Uniform class-balanced is referred as Uniform to save space.
  %  Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy on new, old, and all classes respectively averaged over incremental batches. And $\alpha$ is the final top-1 accuracy on all classes. The $(\uparrow)$ indicates high value is optimum performance.}
  % \label{tab:replay_comp}
  \centering
  \resizebox{\linewidth}{!}{
     %\begin{tabular}{lrrrr}
     \begin{tabular}{lcccc}
     \hline
     Rehearsal Method & $\mu_{N}(\uparrow)$ & $\mu_{O}(\uparrow)$ & $\mu_{A}(\uparrow)$ & $\alpha(\uparrow)$ \\
     \hline
     Offline & --- & --- & --- & $62.12$ \\
     \hline
     Uniform (Latent) & $67.02$ & $69.34$ & $68.95$ & $60.27$ \\
     \textbf{GRASP} (Latent) & $\mathbf{68.25}$ & $\mathbf{70.30}$ & $\mathbf{69.96}$ & $\mathbf{61.99}$ \\
     \hline
     Uniform (Veridical) & $63.62$ & $62.86$ & $62.86$ & $47.98$ \\
     \textbf{GRASP} (Veridical) & $\mathbf{64.06}$ & $\mathbf{63.40}$ & $\mathbf{63.41}$ & $\mathbf{49.31}$ \\
     \hline
    \end{tabular}
    }
  \caption{
   \textbf{Memory $\&$ Compute-Constrained CL.} Comparison between GRASP and uniform class-balanced rehearsals in compute and memory constrained class incremental learning on \textbf{ImageNet-1K}. Uniform class-balanced is referred as Uniform to save space.
   Here $\mu_{N}$, $\mu_{O}$, and $\mu_{A}$ denote top-1 accuracy on new, old, and all classes respectively averaged over incremental batches. And $\alpha$ is the final top-1 accuracy on all classes. The $(\uparrow)$ indicates high value is optimum performance.}
  \label{tab:replay_comp}
\end{table}
